Evaluating the Efficacy of Vectocardiographic and ECG Parameters for Efficient Tertiary Cardiology Care Allocation Using Decision Tree Analysis

Use real word data to evaluate the performance of the electrocardiographic markers of GEH as features in a machine learning model with Standard ECG features and Risk Factors in Predicting Outcome of patients in a population referred to a tertiary cardiology hospital. Patients forwarded to specific evaluation in a cardiology specialized hospital performed an ECG and a risk factor anamnesis. A series of follow up attendances occurred in periods of 6 months, 12 months and 15 months to check for cardiovascular related events (mortality or new nonfatal cardiovascular events (Stroke, MI, PCI, CS), as identified during 1-year phone follow-ups. The first attendance ECG was measured by a specialist and processed in order to obtain the global electric heterogeneity (GEH) using the Kors Matriz. The ECG measurements, GEH parameters and risk factors were combined for training multiple instances of XGBoost decision trees models. Each instance were optmized for the AUCPR and the instance with higher AUC is chosen as representative to the model. The importance of each parameter for the winner tree model was compared to better understand the improvement from using GEH parameters. The GEH parameters turned out to have statistical significance for this population specially the QRST angle and the SVG. The combined model with the tree parameters class had the best performance. The findings suggest that using VCG features can facilitate more accurate identification of patients who require tertiary care, thereby optimizing resource allocation and improving patient outcomes. Moreover, the decision tree model's transparency and ability to pinpoint critical features make it a valuable tool for clinical decision-making and align well with existing clinical practices.

==> Tabelas/TabelaDados.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{landscape}
\begin{table}[]
\resizebox{.85\paperheight}{.4\paperwidth}{%
\large
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
 &
  Parameters &
  Gain &
  Frequency &
  Cover &
  AUC (\%) &
  Threshold &
  Precision (\%) &
  Accuracy (\%) &
  Sensitivy (\%) &
  Specificity (\%) &
  F1-Score \\ \hline
 &
  QRSi &
  0.14 &
  0.14 &
  0.17 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  Qti &
  0.18 &
  0.18 &
  0.13 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  QTc &
  0.12 &
  0.13 &
  0.12 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  Pi &
  0.17 &
  0.14 &
  0.19 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  Pri &
  0.11 &
  0.14 &
  0.10 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  FC &
  0.09 &
  0.10 &
  0.08 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  SAQRS &
  0.15 &
  0.14 &
  0.13 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
\multirow{-8}{*}{Standard ECG parameters} &
  SAT &
  0.12 &
  0.14 &
  0.18 &
  \multirow{-8}{*}{62.3} &
  \multirow{-8}{*}{0.31} &
  \multirow{-8}{*}{66.67} &
  \multirow{-8}{*}{66.27} &
  \multirow{-8}{*}{30.30} &
  \multirow{-8}{*}{66.18} &
  \multirow{-8}{*}{0.42} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Angle QRST &
  0.09 &
  0.13 &
  0.08 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  SVG Elevation Angle &
  0.24 &
  0.23 &
  0.24 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  SVG Azimuth Angle &
  0.28 &
  0.24 &
  0.25 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  SVG Magnitude &
  0.17 &
  0.20 &
  0.19 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\multirow{-5}{*}{\cellcolor[HTML]{EFEFEF}GEH parameters} &
  AUC QT &
  0.23 &
  0.20 &
  0.24 &
  \multirow{-5}{*}{\cellcolor[HTML]{EFEFEF}64.5} &
  \multirow{-5}{*}{\cellcolor[HTML]{EFEFEF}0.44} &
  \multirow{-5}{*}{\cellcolor[HTML]{EFEFEF}53.33} &
  \multirow{-5}{*}{\cellcolor[HTML]{EFEFEF}69.88} &
  \multirow{-5}{*}{\cellcolor[HTML]{EFEFEF}30.77} &
  \multirow{-5}{*}{\cellcolor[HTML]{EFEFEF}73.53} &
  \multirow{-5}{*}{\cellcolor[HTML]{EFEFEF}0.39} \\ \hline
 &
  Previous cardiac surgery &
  0.09 &
  0.19 &
  0.12 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  Previous MI &
  0.35 &
  0.14 &
  0.20 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  Previous PCI &
  0.05 &
  0.16 &
  0.13 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  Previous stroke &
  0.05 &
  0.14 &
  0.13 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  Hypertension &
  0.05 &
  0.10 &
  0.09 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  CKD &
  0.05 &
  0.11 &
  0.08 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  Dialysis &
  0.00 &
  0.00 &
  0 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
\multirow{-8}{*}{Risk factors} &
  Diabetes &
  0.36 &
  0.15 &
  0.24 &
  \multirow{-8}{*}{66.6} &
  \multirow{-8}{*}{0.42} &
  \multirow{-8}{*}{73.33} &
  \multirow{-8}{*}{66.27} &
  \multirow{-8}{*}{31.43} &
  \multirow{-8}{*}{64.71} &
  \multirow{-8}{*}{0.44} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  QRSi &
  0.08 &
  0.13 &
  0.13 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Qti &
  0.14 &
  0.10 &
  0.08 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  QTc &
  0.07 &
  0.14 &
  0.11 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Pi &
  0.13 &
  0.11 &
  0.11 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Pri &
  0.03 &
  0.09 &
  0.05 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  FC &
  0.07 &
  0.07 &
  0.08 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  SAQRS &
  0.04 &
  0.06 &
  0.03 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  SAT &
  0.10 &
  0.11 &
  0.08 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Previous cardiac surgery &
  0.01 &
  0.01 &
  0.00 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Previous MI &
  0.12 &
  0.05 &
  0.08 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Previous PCI &
  0.07 &
  0.04 &
  0.10 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Previous stroke &
  0 &
  0.00 &
  0.00 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Hypertension &
  0 &
  0 &
  0 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  CKD &
  0 &
  0 &
  0 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Dialysis &
  0 &
  0 &
  0 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\multirow{-16}{*}{\cellcolor[HTML]{EFEFEF}Standard ECG + Risk factors} &
  Diabetes &
  0.1 &
  0.07 &
  0.15 &
  \multirow{-16}{*}{\cellcolor[HTML]{EFEFEF}69.2} &
  \multirow{-16}{*}{\cellcolor[HTML]{EFEFEF}0.70} &
  \multirow{-16}{*}{\cellcolor[HTML]{EFEFEF}46.67} &
  \multirow{-16}{*}{\cellcolor[HTML]{EFEFEF}79.52} &
  \multirow{-16}{*}{\cellcolor[HTML]{EFEFEF}43.75} &
  \multirow{-16}{*}{\cellcolor[HTML]{EFEFEF}86.76} &
  \multirow{-16}{*}{\cellcolor[HTML]{EFEFEF}0.45} \\ \hline
 &
  QRSi &
  0.12 &
  0.08 &
  0.09 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  Qti &
  0.05 &
  0.08 &
  0.05 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  QTc &
  0.05 &
  0.07 &
  0.06 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  Pi &
  0.05 &
  0.06 &
  0.06 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  Pri &
  0.08 &
  0.11 &
  0.09 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  FC &
  0.04 &
  0.04 &
  0.03 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  SAQRS &
  0.03 &
  0.06 &
  0.03 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  SAT &
  0.08 &
  0.08 &
  0.07 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  Angle QRST &
  0.02 &
  0.04 &
  0.02 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  SVG Elevation Angle &
  0.10 &
  0.11 &
  0.13 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  SVG Azimuth Angle &
  0.11 &
  0.08 &
  0.13 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
 &
  SVG Magnitude &
  0.1 &
  0.11 &
  0.10 &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-5}
\multirow{-13}{*}{Standard ECG + GEH parameters} &
  AUC QT &
  0.15 &
  0.08 &
  0.15 &
  \multirow{-13}{*}{64.2} &
  \multirow{-13}{*}{0.10} &
  \multirow{-13}{*}{93.33} &
  \multirow{-13}{*}{46.99} &
  \multirow{-13}{*}{24.56} &
  \multirow{-13}{*}{36.76} &
  \multirow{-13}{*}{0.39} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  QRSi &
  0.03 &
  0.06 &
  0.04 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Qti &
  0.07 &
  0.09 &
  0.05 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  QTc &
  0.03 &
  0.04 &
  0.03 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Pi &
  0.09 &
  0.07 &
  0.08 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Pri &
  0.03 &
  0.06 &
  0.04 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  FC &
  0.04 &
  0.04 &
  0.04 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  SAQRS &
  0.04 &
  0.07 &
  0.06 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  SAT &
  0.07 &
  0.08 &
  0.06 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Angle QRST &
  0 &
  0.01 &
  0.01 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  SVG Elevation Angle &
  0.14 &
  0.13 &
  0.16 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  SVG Azimuth Angle &
  0.10 &
  0.10 &
  0.09 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  SVG Magnitude &
  0.04 &
  0.05 &
  0.04 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  AUC QT &
  0.02 &
  0.05 &
  0.05 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Previous cardiac surgery &
  0 &
  0 &
  0 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Previous MI &
  0.12 &
  0.04 &
  0.10 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Previous PCI &
  0.03 &
  0.03 &
  0.07 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Previous stroke &
  0 &
  0 &
  0 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Hypertension &
  0 &
  0.01 &
  0 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  CKD &
  0 &
  0 &
  0 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} &
  Dialysis &
  0 &
  0 &
  0 &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} &
  \cellcolor[HTML]{EFEFEF} \\ \cline{2-5}
\rowcolor[HTML]{EFEFEF} 
\multirow{-21}{*}{\cellcolor[HTML]{EFEFEF}Standard ECG + GEH parameters + Risk factors} &
  Diabetes &
  0.10 &
  0.05 &
  0.10 &
  \multirow{-21}{*}{\cellcolor[HTML]{EFEFEF}75.4} &
  \multirow{-21}{*}{\cellcolor[HTML]{EFEFEF}0.26} &
  \multirow{-21}{*}{\cellcolor[HTML]{EFEFEF}73.33} &
  \multirow{-21}{*}{\cellcolor[HTML]{EFEFEF}69.88} &
  \multirow{-21}{*}{\cellcolor[HTML]{EFEFEF}34.38} &
  \multirow{-21}{*}{\cellcolor[HTML]{EFEFEF}69.12} &
  \multirow{-21}{*}{\cellcolor[HTML]{EFEFEF}0.47} \\ \hline
\end{tabular}
}
\label{TabelaDados}
\end{table}
\end{landscape}
